Efficient Diffusion-Driven Corruption Editor for Test-Time Adaptation

Test-time adaptation (TTA) addresses the unforeseen distribution shifts occurring during test time. In TTA, performance, memory consumption, and time consumption are crucial considerations. A recent diffusion-based TTA approach for restoring corrupted images involves image-level updates. However, using pixel space diffusion significantly increases resource requirements compared to conventional model updating TTA approaches, revealing limitations as a TTA method. To address this, we propose a novel TTA method that leverages an image editing model based on a latent diffusion model (LDM) and fine-tunes it using our newly introduced corruption modeling scheme. This scheme enhances the robustness of the diffusion model against distribution shifts by creating (clean, corrupted) image pairs and fine-tuning the model to edit corrupted images into clean ones. Moreover, we introduce a distilled variant to accelerate the model for corruption editing using only 4 network function evaluations (NFEs). We extensively validated our method across various architectures and datasets including image and video domains. Our model achieves the best performance with a 100 times faster runtime than that of a diffusion-based baseline. Furthermore, it is three times faster than the previous model updating TTA method that utilizes data augmentation, making an image-level updating approach more feasible.

==> paper/backup.tex <==
\section{Introduction}
TTA 모델들이 각광을 받고있다

unseen data stream에 대한 model update가 필요한 경우가 많다 - 자율주행

기존 classifier update 방법론들이 주류 / dataset-level에서 explicit하게 instance-level로 업데이트하는 방법론들은 거의 없다. 이유는, test-time에 데이터셋 업데이틀 할 때 디퓨전 모델들로 많이 하는데, inference time이 굉장히 오래 걸리기 때문이다. 이런 속도에 대한 bottleneck은 생성 모델의 TTA 적용에 있어서 큰 제한이 된다. 

diffusion model의 in-domain editing 성능은 많은 preminary work들에 대해서 검증되어왔다. 여러 supervised training 시나리오에 대해서, unet fine-tuning 혹은 adapter tuning을 통해, auxiliary image condition을 받아 controled image edting을 하는 여러 모델들이 존재한다. 하지만, clean 데이터 manifold에서만 학습된 모델은 online으로 test-time에 unknown corruption이 이 들어오는 TTA 상황에서는 zero-shot diffusion model의 성능에 bottleneck이 존재한다. 이는 corruption에서 clean으로 보내는 direction에 대한 학습이 부재학기에 이를 위한 further training이 필요하다는 점을 시사한다.

% , 대부분의 모델은 pre-training phase에서 이를 고려하지 않기에 여러 adversarial attack 등에 취약하다는 것이 알려져 있다. 
기존에 image restoration 분야애서는, zero-shot 모델을 사용할 경우에는 blur kernel과 같은 degradation matrix를 restoration 시에 가지고 있어야 하기 때문에, unknown corruption에 대한 restoration이 제한된다. 이를 해결하기 위해 몇몇 연구에서는 paired data가 동시에 존재하는 경우에 대해서 corruption modeling을 위한 학습을 진행했다. 하지만 이는 pre-defined corruption에 대해서 paired data의 확보가 필요하며 이는 harsh한 condition이며 labor intensive한 data collection을 요구하게 된다. 또한 이러한 데이터셋에 대한 제약은 task-specific in-domain corruption에 대한 성능은 확보할 수 있으나, diverse한 unseen corruption에 대한 고려는 블기능하다. 

이를 해결하기 위해, 이와는 다른 접근 방식으로, 우리는 data augmentation의 관점에서 새로운 시각을 제안한다. pixmix는 fractal과 같이, 자연에 존재하는 complex한 이미지를 기반으로 data augmentation을 수행하여 classifier의 pre-training 시에 clean image에 대한 accuracy를 잃지 않으면서 robustness를 쉽게 확보할 수 있는 방법이다. 이렇게 얻은 data augmentation을 corruption modeling으로 간주하고, 이를 활용하여 diffusion model을 clean-corruption image pair가 없는 상황에서도 unet fine-tuning을 진행하였다. 
% corrupted 데이터를 clean 데이터로 revert시켜주는 우리는 이러한 기존 방법의 한계를 해결하기 위해, unet fine-tuning을 진행하였다. 

따라서, 이 논문에서 우리는 모델링된 corrupted 데이터를 가지고 augmentation consistency를 가지도록 training을 진행하여 diffusion model의 corruption에 대한 robustness를 높임으로서 out-of-domain corruption에 대한 data reversion 성능을 증가시키는 것을 목적으로 한다. corruption modeling time에서는 class-agnostic한 augmentation을 통해 image의 semantic에 구애받지 않도록 하고, 어떤 corruption이든 clean한 source data로 revert할 수 있도록 many-to-one 모델링을 가능하도록 하기 위해 diffusion model의 unet fine-tuning을 진행하였다. 

% 먼저, instruct-pix2pix 모델은 stable diffusion 기반이고, 8-channel Unet을 활용하여 image condition을 받는 모델이다. 
% 

우리는 image editing에서 자주 사용되는 stable diffusion v1.5 모델~\cite{rombach2022high}을 사용하였고, image를 condition으로 받는 image editing 모델인 instruct-pix2pix~\cite{brooks2023instructpix2pix} 모델을 활용하였다. 그리고 이를 imagenet에 튜닝하여 dataset bias를 완화하는 과정을 수행한 후 다양한 TTA 시나리오에서 dataset update가 classifier의 성능에 미치는 영향을 확인하였다.

우리의 방법은 기존의 text-guided 세팅(image-text paired)과 달리, 어떤 이미지가 들어오든지 clean한 이미지로 dataset을 update하기 위해 training/inference time 시에 동일한 text를 활용한다. To be specific, 'Clean the image'라는 instruction text를 fix하여 many-to-one reverting direction을 학습하도록 하였다. 따라서, 이를 통해 classifier-free guidance를 기반으로 image editing을 하는 방식을 가능하도록 한다. 

우리는 IP2P 기반 DPM 모델 (약 20 NFEs), 그리고 해당 모델로부터 distillation을 수행한 LCM 모델 (약 4 NFEs)의 두 가지의 버전을 제안하였고, 다양한 downstream task에 적용하여 성능을 검증하였다. 우리는 evaluation protocol에 맞춰 imagenet-c, c-bar 데이터셋을 활용하여 모델의 성능을 검증하였으며 우리의 제안하는 LCM 모델을 통해 corrupted video도 reversion하여 성능에 기여할 수 있음을 보였다. 

% 우리는 instruction을 기반으로 image editing이 가능하도록 하기 워해, instruct pix2pix 모델을 활용한다. 
% 이를 위해, 
% inference time에 어떤 corruption이 들어오든지 
% 우리는 stable diffusion v1.5 모델을 활용하였고,  


==> paper/tabs/tab4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\hline
Corruptions & gauss & pepper & salt & shot & zoom & impulse & defocus & motion & jpeg & contrast & rain & h265.abr & avg \\
\hline
Source-Only & 17.92 & 23.66 & 7.85 & 72.48 & 76.04 & 17.16 & 37.51 & 54.51 & 83.40 & 62.68 & 81.44 & 81.58 & 51.35 \\
NORM & 45.23 & 42.43 & 27.91 & 86.25 & 84.43 & 46.31 & 54.32 & 64.19 & 89.19 & 75.26 & 90.43 & 83.27 & 65.77 \\
DUA & 36.61 & 33.97 & 22.39 & 80.25 & 77.13 & 36.72 & 44.89 & 55.67 & 85.12 & 30.58 & 82.66 & 78.14 & 55.34 \\
TENT & 58.34 & 53.34 & 35.77 & 89.61 & 87.68 & 59.08 & 64.92 & 75.59 & 90.99 & 82.53 & 92.12 & 85.09 & 72.92 \\
SHOT & 46.10 & 43.33 & 29.50 & 85.51 & 82.95 & 47.53 & 53.77 & 63.37 & 88.69 & 73.30 & 89.82 & 82.66 & 65.54 \\
T3A & 19.35 & 26.57 & 8.83 & 77.19 & 79.38 & 18.64 & 40.68 & 58.61 & 86.12 & 67.22 & 84.0 & 83.45 & 54.17 \\
Ours & 19.35 & 26.57 & 8.83 & 77.19 & 79.38 & 18.64 & 40.68 & 58.61 & 86.12 & 67.22 & 84.0 & 83.45 & 54.17 \\
\hline 
ViTTA & 71.37 & 64.55 & 45.84 & 91.44 & 87.68 & 71.90 & 70.76 & 80.32 & 91.70 & 86.78 & 93.07 & 84.56 & 78.33 \\
\rowcolor{LightCyan}
+ Ours & 71.37 & 64.55 & 45.84 & 91.44 & 87.68 & 71.90 & 70.76 & 80.32 & 91.70 & 86.78 & 93.07 & 84.56 & 78.33\\
\hline
\end{tabular}
}
\caption{. Top-1 Classification Accuracy (\%) for all corruptions in the UCF101 dataset, while using the TANet backbone. DUA is evaluated with batch size of 1, following the setting in the original work [30]. All the other methods are evaluated with batch size of 8.}
\label{table:performance_metrics}
\end{table}


==> paper/tabs/tab_detail.tex <==
\begin{table*}[t]
    % \vspace{-0.15in}
    \caption{Comparisons with baselines on ImageNet-C at severity level 5 under a mild scenario regarding accuracy (\%). The \textbf{bold} value signifies the top-performing result.}
    % \vspace{-0.18in}
    \label{tab:imagenet-c-detail}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
 \begin{center}
  \begin{threeparttable}
 \LARGE
    \resizebox{1.0\linewidth}{!}{
 	\begin{tabular}{l|ccc|cccc|cccc|cccc|c}
 	\multicolumn{1}{c}{} & \multicolumn{3}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital}  \\
 	  & Gauss. & Shot & Impul. & Defoc. & Glass & Motion & Zoom & Snow & Frost & Fog & Brit. & Contr. & Elastic & Pixel & JPEG & Avg.  \\
    \cmidrule{1-17}
        ResNet-50-BN & 2.2                        & 2.9                      & 1.8                        & 17.9                       & 9.8                       & 14.8                       & 22.5                     & 16.9                     & 23.3                      & 24.4                    & 58.9                      & 5.4                        & 16.9                        & 20.7                      & 31.7                     & 18.0  \\ 
        ~~$\bullet~$MEMO & 7.5                       & 8.8                     & 8.9                       & 19.8                       & 13.0                      & 20.7                       & 27.7                     & 25.3                     & 28.7                      & 32.2                    & 61.0                      & 11.0                       & 23.8                        & 33.0                      & 37.6                     & 23.9  \\
        ~~$\bullet~$DDA (\textcolor{red}{SAR report}) & 32.2                       & 33.1                     & 32.0                       & 14.6                       & 16.4                      & 16.6                       & 24.4                     & 20.0                     & 25.5                      & 17.2                    & 52.2                      & 3.2                       & 35.7                        & 41.8                      & 45.4                     & 27.2  \\
        \rowcolor{cyan!10}~~$\bullet~$Ours (DPM) & 38.3                       & 40.8                     & 37.9                       & 26.2                       & 10.5                      & 14.1                       & 22.5                     & 39.8                     & 36.4                      & 35.1                    & 59.9                      & 25.7                       & 24.3                        & 21.9                      & 34.3                     & \textbf{31.2}  \\ 
        \rowcolor{cyan!10}~~$\bullet~$Ours (CM) & -                       & -                     & -                       & -                       & -                      & -                       & -                     & -                     & -                      & -                    & -                      & -                       & -                        & -                      & -                     & - \\ 
        % \rowcolor{cyan!10}~~$\bullet~$DeYO (ours) & \textbf{35.6$_{\pm0.2}$}                       & \textbf{37.9$_{\pm0.1}$}                     & \textbf{37.1$_{\pm0.1}$}                       & \textbf{33.8$_{\pm0.2}$}                       & \textbf{34.1$_{\pm0.2}$}                      & \textbf{48.5$_{\pm0.1}$}                       & \textbf{52.8$_{\pm0.1}$}                     & \textbf{52.7$_{\pm0.0}$}                     & \textbf{46.4$_{\pm0.1}$}                      & \textbf{60.6$_{\pm0.0}$}                    & {68.0$_{\pm0.1}$}                      & \textbf{46.1$_{\pm0.1}$}                       & \textbf{58.4$_{\pm0.1}$}                        & \textbf{61.5$_{\pm0.1}$}                      & \textbf{55.7$_{\pm0.1}$}                    & \textbf{48.6$_{\pm0.0}$}  \\ 
	\end{tabular} 
        }
    \end{threeparttable}
    \end{center}
% \vspace{-0.13in}
\end{table*}
